MerLin: A Discovery Engine for Photonic and Hybrid Quantum Machine Learning

Identifying where quantum models may offer practical benefits in near term quantum machine learning (QML) requires moving beyond isolated algorithmic proposals toward systematic and empirical exploration across models, datasets, and hardware constraints. We introduce MerLin, an open-source framework designed as a discovery engine for photonic and hybrid quantum machine learning. MerLin integrates optimized strong simulation of linear optical circuits into standard PyTorch and scikit learn workflows, enabling end-to-end differentiable training of quantum layers. MerLin is designed around systematic benchmarking and reproducibility. As an initial contribution, we reproduce eighteen state-of-the-art photonic and hybrid QML works spanning kernel methods, reservoir computing, convolutional and recurrent architectures, generative models, and modern training paradigms. These reproductions are released as reusable, modular experiments that can be directly extended and adapted, establishing a shared experimental baseline consistent with empirical benchmarking methodologies widely adopted in modern artificial intelligence. By embedding photonic quantum models within established machine learning ecosystems, MerLin allows practitioners to leverage existing tooling for ablation studies, cross-modality comparisons, and hybrid classical-quantum workflows. The framework already implements hardware-aware features, allowing tests on available quantum hardware while enabling exploration beyond its current capabilities, positioning MerLin as a forward-looking co-design tool linking algorithms, benchmarks, and hardware.

==> Sections/Future_proofing.tex <==
\subsubsection{Quantum Bridge}
Qubit-based platforms (PennyLane, Qiskit, Cirq) operate in a $2^n$-dimensional computational basis, while photonic systems operate in Fock space, a combinatorially different structure. MerLin's \texttt{QuantumBridge} provides a differentiable qubit-to-photonic interface, enabling hybrid workflows that combine qubit-based variational circuits with photonic quantum layers.
The standard mapping uses \emph{dual-rail encoding}, where each qubit is represented by one photon across two modes. \texttt{MerLin} extends this to arbitrary \emph{qudit/qubit mappings} following the QLOQ scheme~\cite{lysaght2024quantumcircuitcompressionusing}, reducing the photon count required to encode the same logical space.
The \texttt{QuantumBridge} integrates with standard PyTorch workflows:
\begin{codecellT}[QuantumBridge Usage] 
from merlin.bridge import QuantumBridge
from merlin import QuantumLayer, MeasurementStrategy
 
# Bridge: 2 qubits -> 2 photons, 4 modes (dual-rail)
bridge = QuantumBridge(
    n_photons=2, n_modes=4,
    qubit_groups=[1, 1],
    computation_space=ComputationSpace.UNBUNCHED
)
 
# Compose with upstream qubit circuit and downstream photonic layer
model = torch.nn.Sequential(qubit_circuit, bridge, merlin_layer)
\end{codecellT}

\subsubsection{Quantum Memristor (Neuromorphic Components)}
A memristor is a circuit element whose resistance depends on the history of current flow, mimicking synaptic plasticity. The photonic analogue is a Mach-Zehnder interferometer with a feedback loop, where the internal phase is updated based on detection statistics~\cite{spagnolo2022experimental, selimovic_experimental_2025}. This feedback provides the memory and nonlinearity required for tasks like time-series prediction.

\subsubsection{Future Integrations}
The bridge architecture could link any quantum computing platform that produces statevectors to \texttt{MerLin}. A potential direction is integration with continuous-variable systems such as Strawberry Fields. For the memristive phase shifter, which can already be constructed in \texttt{MerLin}, we plan to provide more direct support in the \texttt{CircuitBuilder}.
